Towards 4D Human Video Stylization

We present a first step towards 4D (3D and time) human video stylization, which addresses style transfer, novel view synthesis and human animation within a unified framework. While numerous video stylization methods have been developed, they are often restricted to rendering images in specific viewpoints of the input video, lacking the capability to generalize to novel views and novel poses in dynamic scenes. To overcome these limitations, we leverage Neural Radiance Fields (NeRFs) to represent videos, conducting stylization in the rendered feature space. Our innovative approach involves the simultaneous representation of both the human subject and the surrounding scene using two NeRFs. This dual representation facilitates the animation of human subjects across various poses and novel viewpoints. Specifically, we introduce a novel geometry-guided tri-plane representation, significantly enhancing feature representation robustness compared to direct tri-plane optimization. Following the video reconstruction, stylization is performed within the NeRFs' rendered feature space. Extensive experiments demonstrate that the proposed method strikes a superior balance between stylized textures and temporal coherence, surpassing existing approaches. Furthermore, our framework uniquely extends its capabilities to accommodate novel poses and viewpoints, making it a versatile tool for creative human video stylization.

==> method_copy.tex <==

\section{Methodology}
\vspace{-2mm}
\label{sec:algorithm}

\begin{figure*}[t]
% \vspace{-6mm}
\centering
\includegraphics[width=1\linewidth]{./imgs/framework.pdf}
% \end{tabular}
\vspace{-4mm}
\caption{\textbf{Overview.} 
Given a camera ray, we sample foreground (human) and background points separately through the human and scene NeRFs. 
%
The points from the human are warped into canonical space via inverse warping. Then, features for each point are derived from the triplane representation via bilinear interpolation on three 2D planes, incorporated by Hadamard product, and utilized to predict the RGB and density. We composite the foreground and background points for the dynamic foreground and multi-view background along each camera ray and apply volume rendering to attain the pixel feature on the 2D feature map. Subsequently, stylization is implemented on the feature map by AdaAttN~\citep{liu2021adaattn}, and a decoder then processes the stylized feature to predict the stylized image. Our model can stylize novel views and animated humans in the same scene by giving the novel camera parameters and articulation as the input.
}
\label{fig:pipeline}
% \vspace{-10mm}
\vspace{-4mm}
\end{figure*}




% \subsection{Overview}
Given a monocular video of a dynamic human and an arbitrary style image, our goal is to synthesize {\em stylized novel views} of a person in {\em different poses} (i.e., animated humans) in a scene. To achieve this, we propose a unified framework (Figure.~\ref{fig:pipeline}) consisting of three modules: 1) two novel triplane-based feature representation networks to encode geometric and appearance information of dynamic humans and its surroundings, 2) a style transfer module to modulate the rendered feature maps from NeRFs as conditioned on the input style image, 3) a lightweight decoder to synthesize the stylized images from novel viewpoints or new poses. In this section, we will present these three modules in detail.
%
%To achieve this, as illustrated in our system pipeline (Figure. ~\ref{fig:pipeline}), we encoding geometric and appearance information of a scene through two neural radiance field networks: a human NeRF learns the dynamic human attributes conditioned on the human model prior, and a scene NeRF represents the multi-view background surrounding the human. 
%
%We introduce a novel triplane-based feature representation network in each network to encode the input efficiently. 
%
%For a collection of points sampled along an emitted camera ray, we extract the corresponding features from the triplane module and use them to render a feature map through volume rendering. 
%
%A style transfer module then modulates the feature map, taking the input style image as a condition.
%
%Finally, we apply a CNN decoder to synthesize the stylized images from novel viewpoints or new poses.

\vspace{-2mm}
\subsection{Geometry Guided Tri-plane based Feature Representation}
\vspace{-2mm}
Motivated by~\citep{fridovich2023k}, we propose a tri-plane representation to model each video frame from a scene, thereby reducing memory usage and accelerating the training and rendering processes compared to MLPs. 
%
The tri-plane representation, shown in Figure~\ref{fig:pipeline}, describes a scene with three orthogonal planes $(\textbf{P}_{xy}, \textbf{P}_{xz}, \textbf{P}_{yz})$. 
%
The neural
radiance density and appearance of a point are obtained by projecting its 3D coordinate over three axis-aligned planes and decoding the product of three bilinearly interpolated features with a tiny MLP.  
%
\textbf{(not clear? what is expressiveness???)} However, triplane is limited
in expressiveness when directly optimized using the reconstruction loss between the inputs and the rendered RGB values. 
%
To overcome this limitation, we propose to encode the 3D coordinates anchored to the triplane as the geometric prior over the whole space. 
%
Here we discretize the 3D space as a volume and divide it into small voxels, with each voxel size of 10mm $\times$ 10mm $\times$ 10mm. 
%
Voxel coordinates transformed by the positional encoding $\gamma_v(\cdot)$ are mapped onto three planes to serve as the tri-plane input. 
%
Features projected onto the same pixel are aggregated using average
pooling operation, resulting in planar features with size $H_{\textbf{P}_i} \times W_{\textbf{P}_i} \times D$, where $D$ is the dimension of the feature on each plane.
%
Similar to the U-Net architecture~\citep{ronneberger2015u},
we use three encoders with 2D convolutional networks to encode the tri-plane features. As shown in Figure~\ref{fig:triplane_our}, the proposed geometry guided tri-plane produces more clear background prediction than direct optimization of the tri-plane, owing to the more robust feature representation.

\begin{figure*}[t]
% \vspace{-6mm}
\centering
\includegraphics[width=0.8\linewidth]{imgs/triplane_our.pdf}
% \end{tabular}
\vspace{-3mm}
\caption{\textbf{Visual benefits} between direct optimization of the tri-plane feature and our proposed geometry guided tri-plane feature.
}
\label{fig:triplane_our}
% \vspace{-10mm}
\vspace{-3mm}
\end{figure*}
%
%Here, skip connections are removed, and a bilinear up-sampling operation is adopted at the entry of each stage.

% We query any 3D spatial point by projecting it onto each triplane, retrieving the corresponding feature vector by bilinear interpolation.

To obtain the feature $f_p(\bm{x})$ of a 3D point $\bm{x} = (x, y, z)$, we project the point onto three planes $\pi_p(\bm{x})$, $p\in (\textbf{P}_{xy}, \textbf{P}_{xz}, \textbf{P}_{yz})$, 
where $\pi_p$ presents the projection operation that maps $\bm{x}$ onto the $p$'th plane. 
%
Then, bilinear interpolation of a point is executed on a regularly spaced 2D grid to obtain the feature vector by $\phi(\pi_p(\bm{x}))$. 
%
The operation of each plane is repeated to obtain three feature vectors $f_p(\bm{x})$.
%
To incorporate these features over three planes, we use the Hadamard product (element-wise multiplication) to produce an integrated feature vector,
\begin{equation}
f(\bm{x}) = \prod_{p\in (\textbf{P}_{xy}, \textbf{P}_{xz}, \textbf{P}_{yz})} f_p(\bm{x}).
\label{equ:tri_agg}
\end{equation}
%
Finally,  $f(\bm{x})$ will be decoded into color and density using two separate MLPs aggregated by volume rendering. 
%
Either Hadamard product or additional operations can be utilized to
generate the feature vector $f(\bm{x})$.
%
We choose the Hadamard product here as it can generate spatially localized signals, which is a distinct advantage over addition, as described in~\citep{fridovich2023k}.

\vspace{-2mm}
\subsection{Neural Radiance Fields}
\label{sec:nerfs}
\vspace{-2mm}
We propose leveraging the neural volumetric field to model 3D scenes and stylized 2D feature representations rendered by NeRFs. 
%
Specifically, we extend the original NeRF~\citep{mildenhall2020nerf} that outputs the color for each point on the camera ray to predict the $C$-dimensional feature vector~\( \hat{f}(\bm{x}) \in \mathbb{R}^C \). 
%
For every queried point \( \bm{x} \in \mathbb{R}^3 \), our model learns the volume density \(\sigma\) and feature vector~\( \hat{f}(\bm{x})\) by
\begin{equation}
F_{\Theta}:(f(\bm{x}), \gamma_d({\bm d})) \rightarrow (\sigma, \hat{f}(\bm{x})),
\end{equation} 
where $\gamma_d({\bm d})$ represents the positional encoding on the view direction $\bm d$ and $f(\bm{x})$ is the feature vector produced by the triplane. 
%
Then, the feature vector of any given pixel is derived by accumulating all $N$ sampled points along the ray $\bm{r}$ through integration~\citep{mildenhall2020nerf}:
\begin{equation}
f(\bm{r}) = \sum_{i=1}^N w_i \hat{f}(\bm{x_i}),
\quad w_i = T_i \left( 1-\mathrm{exp}\left( -\sigma_i \delta_i \right) \right),
\label{eq:volumerender}
\end{equation}
where $\sigma_j$ and $\delta_i$ denote the volume density and distance between adjacent samples, 
\(w_i\) is the weight of the feature vector $\hat{f}(\bm{x_i})$ on the ray \(\bm{r}\),  and $T_i=\exp(-\sum_{j=1}^{i-1}\sigma_i \delta_i)$ is the accumulated transmittance along the ray.
%
We treat the backgrounds across frames as multi-view images and train the scene NeRF for the background model with the human masked out in each frame. 
%
To capture dynamic humans with various poses, we train the human NeRF in the canonical space, leveraging priors with the deformation field by transforming the human from observation to canonical space. 
%
Here, the observation space describes the images from the input video, and the canonical space is the static one shared by all frames.

%\textbf{Scene NeRF}
\vspace{-4mm}
\paragraph{Scene NeRF.} We extract features from the background triplane to predict the density and feature vector $\hat{f}_b(\bm{x})$ for each point using two MLPs.
%
The density branch adopts one fully-connected layer, while the feature branch utilizes a hidden layer comprising 128 units, followed by an output layer. 
%
Subsequently, the feature vectors on the same camera ray are aggregated to generate a single feature vector $f_b(\bm{r})$ for each pixel using Equation~\ref{eq:volumerender}.

%\textbf{Human NeRF}. 
\vspace{-4mm}
\paragraph{Human NeRF.} To synthesize a pixel on the human body within the observation space for each frame, we optimize the NeRF in the canonical space where points along the corresponding ray are transformed from the observation space by the rigid transformation associated with the closest point on the mesh. 
%
We use a parametric SMPL~\citep{loper2015smpl} model to provide explicit guidance on the deformation of spatial points. 
%
This approach is beneficial for learning a meaningful canonical space while simultaneously reducing dependency on diverse poses when generalized to unseen poses. 
%
This allows us to train the NeRF within dynamic scenarios featuring a moving person and animate the same person during inference.

Motivated by~\citep{chen2021animatable}, the template pose is defined as X-pose $\theta_{c}$ because of its good visibility and separability for each body component in the canonical space.
%
The pose $\theta_{o}$ in the observation space can be converted to X-pose $\theta_{c}$ in the canonical space by using the inversion of the linear skinning derived from the SMPL model.
%
As points within the space near the mesh should correspondingly move with adjacent vertices, we extend these transformation functions to the space surrounding the mesh surface.

Specifically, the inverse linear blend skinning is defined based on the 3D human skeleton. 
%
The human skeleton represents $K$ parts that generate $K$ transformation matrices $\{G_k\} \in SE(3)$:
\begin{equation}
    \bm{\Tilde x} = \left( \sum_{k=1}^K w_o(\bm x)_k G_k \right)^{-1} \bm{x},
    \label{eq:inverse}
\end{equation}
where $w_o(\bm x)_k$ is the blend weight of the $k$-th part. $\bm{x}$ and $\bm{\Tilde x}$ denotes the observation and canonical points respectively.
%
Equation~\ref{eq:inverse} does not express all details during the warping operation.
%
Thus, motivated by~\citep{jiang2022neuman}, we adopt an error-correction network $\mathcal{E}$ to correct the errors in the warping field, which learns a mapping for a point from the observation space to the canonical space. 
%
Here, $\mathcal{E}$ comprises an MLP with the coordinates as the input and predicts the error. 
%
The canonical point is defined by
\begin{equation}
    \bm{\Tilde x_c} = \bm{\Tilde x} + \mathcal{E}(\bm{x}).
    \label{eq:canonical}
\end{equation}
%
We then adopt Equation~\ref{equ:tri_agg} and~\ref{eq:volumerender} to generate a feature vector $f_h(\bm{r})$ for the pixel on the human.

\vspace{-4mm}
\paragraph{Composite NeRFs.}  To obtain the RGB value for each image pixel, two rays, one for the human NeRF and the other for the scene NeRF, are utilized. 
%
For each ray, we generate the feature vectors $ f_h(\bm{r})$ and $f_b(\bm{r})$ for the sampled human and background points and then incorporate them according to Equation~\ref{eq:volumerender} to produce the rendered feature vector $f_c$.

% The colors and densities are sorted in ascending order based on the depth values, similar to NeuMan~\citep{jiang2022neuman}. 
%
% Finally, we integrate these values to obtain the pixel using Equation~\ref{eq:volumerender}.

\vspace{-2mm}
\subsection{Stylizing the Scene}
\vspace{-2mm}
The stylization module takes features of the style and content images as input and generates the stylized image based on the Adaptive Attention Normalization (AdaAttN) layer~\citep{liu2021adaattn}. 
% to formulate the stylization process given the content and style features, which consist of a VGG encoder, an adaptive instance normalization layer, and a CNN-based decoder. 
%
The feature map of the style image is extracted from the pretrained VGG network~\citep{simonyan2014very}. 
%
Let  $F_{s}$ be the style features and $F_{c}$ be the set of content features tailored to a 2D patch.
%
Here, the feature associated with each pixel is given by Equation~\ref{equ:composite}. 
%
The style transfer module is formulated by 
\begin{equation}
\small
    F_{cs} = \psi(\mbox{AdaAttN}(\phi(F_{c}), F_{s})),
\end{equation}
where $\phi$ and $\psi$, formulated as MLPs, are learned mappings for the content and stylized features, and  $\mbox{AdaAttN}$~\citep{liu2021adaattn} is designed to adaptively transfer the feature distribution from the style image to the content by the attention mechanism. 
%
% Here, $\mbox{AdaAttN}$ computes attention between every content feature and each style feature and uses the attention map to modulate the affine parameters within the instance normalization applied to content features. 
Specifically, $F_{cs}$ is generated by calculating the attention map within the features of the content and style images.
%
%and then normalizing the content feature for per-point feature distribution alignment using the weighted mean and standard variance maps of the style feature. 
%
The stylized feature $F_{cs}$ will then be applied to generate the stylized image via a decoder.

\vspace{-2mm}
\subsection{Image Decoding}
\label{sec:img_decoding}
\vspace{-2mm}
After stylizing the scene, an image decoder is adopted by mapping the 2D feature $F_{cs} \in \mathbb{R}^{H \times W \times M}$ that captures high-level information to the final stylized image $I \in \mathbb{R}^{H \times W \times 3}$ at input resolution by
%\begin{align} 
%\begin{split}
\begin{equation}
F_{\theta}: \mathbb{R}^{H \times W \times M} \to \mathbb{R}^{H \times W \times 3}.
\end{equation}
%\end{split}
%\end{align}
%
The operation $F_{\theta}$ comprised of convolutional and ReLU activation layers, aiming to render a full-resolution RGB image, is parameterized as a 2D decoder.  
%
In the convolutional layer, we opt for $3\times3$ kernel sizes without intermediate layers to only allow for spatially minor refinements to avoid entangling global scene properties during image synthesis.

\vspace{-2mm}
\subsection{Objective Functions}
\vspace{-2mm}
\label{sec:obj_func}
Our goal is to stylize novel views of animated humans based on the reconstructed scene and humans. 
%
We initially train the NeRFs that predict each pixel's RGB values to achieve this. 
%
Following this, we remove the last fully connected layer and introduce a stylization module and a decoder to synthesize stylized images. 
%
Next we introduce the losses adopted for training both the scene and human NeRFs, which is followed by the objectives for stylization.

\vspace{-4mm}
\paragraph{Scene NeRF.} The objective function for training the scene NeRF is defined as 
\begin{equation}
\mathcal{L}_{s}(\bm{r})=\sum_{\bm{r}\in \mathcal{R}}||C_s(\bm{r})-\tiC{s}(\bm{r})||,
\label{eq:scene_rgb}
\end{equation}
where $R$ is the set of rays. $C_s$ and $\Tilde{C}_s$ denote the prediction and the ground truth RGB values. 

\vspace{-4mm}
\paragraph{Human NeRF.} The region covered by the human mask $\Mask(\cdot)$ is optmized by 
\begin{equation}
    \loss{r}(\bm{r}) =  \Mask(\bm{r})
    ||C_h(\bm{r})-\tiC{h}(\bm{r})||,
    \label{eq:human_rgb}
\end{equation}
where $C_h(\bm{r})$ and $\tiC{h}(\bm{r})$ are the rendered and ground truth RGB values.

We use $\loss{a}$ to enforce the accumulated alpha map from the human NeRF to be similar to the detected human mask, 
\begin{equation}
    \loss{a}(\bm{r}) =  \Mask({\bm{r}})
   ||1 - \balpha_h(\bm{r})||,
    \label{eq:human_alpha}
\end{equation}
where $\balpha_h(\cdot)$ corresponds to accumulated density over the ray.

To remove artifacts such as blobs in the canonical space and semi-transparent canonical humans, we enforce the volume $\sigma_h$ inside the canonical SMPL mesh to be solid while enforcing the volume $\sigma_h$ outside the canonical SMPL mesh to be empty:
\begin{equation}
    \loss{smpl}(\bm{\Tilde x}, \sigma_h) =  
    \begin{cases}
        \left\| 1 - \sigma_h \right\|,               & \text{if } \bm{\Tilde x} \text{ inside SMPL mesh}\\
        \lvert \sigma_h \rvert,              & \text{otherwise.}
    \end{cases}
    \;.
    \label{eq:human_smpl}
\end{equation}
This loss function encourages the proposed method to model shapes as solid surfaces (i.e., sharp outside-to-inside transitions).

To encourage the solid surfaces in the canonical human, we encourage the weight of each sample to be either 1 or 0, given by
\begin{equation}
    \loss{hard} = -\log(e^{-|\weight|} + e^{-|1-\weight|}),
    \label{eqn:huamn_hard}
\end{equation}
where $w$ is derived from an accumulation of
the transmittance along the camera ray as defined in Equation~\ref{eq:volumerender}.
%
In addition, a canonical edge loss $\loss{edge}$ is utilized
to predict a sharp canonical shape. 
%
This is carried out by raycasting a random line in the canonical volume and encouraging the alpha $\balpha_c$ values to be 1 or 0:
% However, this penalty alone is insufficient to obtain a sharp canonical shape; we also add a canonical edge loss, $\loss{edge}$. 
% %e, we encourage the accumulated alpha values to be one o by rendering a random straight ray in the canonical volume 0. 
%
\begin{equation}
    \loss{edge} = -\log(e^{-|\balpha_c|} + e^{-|1-\balpha_c|}).
    \label{eqn:human_edge}
\end{equation}
% where $\balpha_c$ is the accumulated alpha value obtained from a random straight ray in canonical space.
%
Overall, the losses for our model are formulated by
\begin{equation}
\begin{split}
    \loss{h} = \loss{r} + \lambda_{a}\loss{a} + \lambda_{smpl}\loss{smpl} + \lambda_{hard}\loss{hard} + \lambda_{edge}\loss{edge}.
    \label{eqn:human_losses}
\end{split}
\end{equation}
% In this project, we will determine the weight factors for the best results. 
we set $\lambda_{mask}=0.01$, $\lambda_{smpl}=1.0$, $\lambda_{hard}=0.1$, and $\lambda_{edge}=0.1$. 
The $\lambda_{mask}$ linearly decays to 0 throughout the training since the detected masks are inaccurate.

After training the scene and humans, we discard the last fully connected layer. Then, the feature vector and density for sampled points are aggregated to render the feature vector as introduced in \textbf{Composite NeRFs} of Section~\ref{sec:nerfs}. 
%
Finally, a decoder with convolutional and nonlinear layers decomposes the feature map to the RGB image. 
%
Here, two losses are applied, aiming to reconstruct the input and acquire semantic information for the feature map introduced in Section~\label{sec:img_decoding},
\begin{equation}
    \loss{v} = ||F_c-\Tilde F_c||+\sum_{l\in l_p}||F^l(I)-F^l(\Tilde I)||+||I - \Tilde I||,
    \label{eqn:vgg_losses}
\vspace{-2mm}
\end{equation}
where $F_c$ and $\Tilde F_c$ denote the rendered feature map and the feature extracted from the pretrained VGG network, $F( I)$ and $F(\Tilde I)$ are the predicted features, and the features extracted from VGG with the RGB image as the input. 
%
In addition, $I$ and $\Tilde I$ are the predicted and ground truth images. $l_p$ denotes the set of VGG layers.  
% utilized to calculate the perceptual loss.

\vspace{-4mm}
\paragraph{Stylization.} We adopt the content and style losses from AdaAttN~\citep{liu2021adaattn}, encompassing both global style loss and local feature loss. The former ensures a global stylized effect, whereas the latter ensures that the feature map of the stylized image aligns with the transformation of the content image.

